Planck 2013 results. XVIII. Gravitational lensing-infrared background correlation

The multi-frequency capability of the Planck satellite provides information both on the integrated history of star formation (via the cosmic infrared background, or CIB) and on the distribution of dark matter (via the lensing effect on the cosmic microwave background, or CMB). The conjunction of these two unique probes allows us to measure directly the connection between dark and luminous matter in the high redshift (1 < z <3) Universe. We use a three-point statistic optimized to detect the correlation between these two tracers. Following a thorough discussion of possible contaminants and a suite of consistency tests, using lens reconstructions at 100, 143 and 217 GHz and CIB measurements at 100-857 GHz, we report the first detection of the correlation between the CIB and CMB lensing. The well matched redshift distribution of these two signals leads to a detection significance with a peak value of 42 \sigma at 545 GHz and a correlation as high as 80% across these two tracers. Our full set of multi-frequency measurements (both CIB auto- and CIB-lensing cross-spectra) are consistent with a simple halo-based model, with a characteristic mass scale for the halos hosting CIB sources of log_{10}(M/M_sun) = 10.5 \pm 0.6. Leveraging the frequency dependence of our signal, we isolate the high redshift contribution to the CIB, and constrain the star formation rate (SFR) density at z>1. We measure directly the SFR density with around 2 sigma significance for three redshift bins between z=1 and 7, thus opening a new window into the study of the formation of stars at early times.

==> PlanckTable.tex <==
%Planck table template file, to be used with A&A style and Planck.tex to produce Planck tables %  for publication.
%
% version 11 September 2011 ---  CRL

\begin{table*}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{}                          % Caption goes here.
\label{}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{                            % Template goes here.
\noalign{\doubleline}
                                    % Table headings go here.
\noalign{\vskip 3pt\hrule\vskip 5pt}
                                    % Body of table goes here.
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
\tablenote a Footnote a.\par
\tablenote b Footnote b.\par
\endgroup
\end{table*}                        % table* is a two-column table.  Drop the * for one column.

